GOTM: a Goal-Oriented Framework for Capturing Uncertainty of Medical Treatments

It has been widely recognized that uncertainty is an inevitable aspect of diagnosis and treatment of medical disorders. Such uncertainties hence, need to be considered in computerized medical models. The existing medical modeling techniques however, have mainly focused on capturing uncertainty associated with diagnosis of medical disorders while ignoring uncertainty of treatments. To tackle this issue, we have proposed using a fuzzy-based modeling and description technique for capturing uncertainties in treatment plans. We have further contributed a formal framework which allows for goal-oriented modeling and analysis of medical treatments.

==> complexity.tex <==
\section{Complexity Analysis}
\label{sec_complexity}

Our employed FIS with $m$ number of fuzzy inputs (prioritization constraints) and $k$ possible values for each variable requires less than $m\times k$ number of comparisons to infer the priority of a single security requirement. Hence, complexity of PPSS to infer priority of $n$ requirements, is of $O(m\times k\times n)$. Given $m$ and $k$ are constant numbers, the complexity of our employed fuzzy inference system belongs to order of  $O(n)$. For three organization constraints of impact, cost and technical-ability, $n\times 3\times 3$ comparisons are required to prioritize the requirements in $SRL[g]$ where $g$ is a security goal in GFG of the system and n denotes the number of requirements in $SRL[g]$. If performed for all security goals in SRL of the system, PPSS prioritization can be as complex as $O(m\times k\times n\times n)=O(n^2)$.

==> related.tex <==
\section{Related Work}




